Minimizing the Age of Information in Wireless Networks with Stochastic Arrivals

We consider a wireless network with a base station serving multiple traffic streams to different destinations. Packets from each stream arrive to the base station according to a stochastic process and are enqueued in a separate (per stream) queue. The queueing discipline controls which packet within each queue is available for transmission. The base station decides, at every time t, which stream to serve to the corresponding destination. The goal of scheduling decisions is to keep the information at the destinations fresh. Information freshness is captured by the Age of Information (AoI) metric. In this paper, we derive a lower bound on the AoI performance achievable by any given network operating under any queueing discipline. Then, we consider three common queueing disciplines and develop both an Optimal Stationary Randomized policy and a Max-Weight policy under each discipline. Our approach allows us to evaluate the combined impact of the stochastic arrivals, queueing discipline and scheduling policy on AoI. We evaluate the AoI performance both analytically and using simulations. Numerical results show that the performance of the Max-Weight policy is close to the analytical lower bound.

==> body/11_appD_OptimalRand.tex <==
\section{Proof of Theorem \ref{theo.scheduling_policy_OptimalBuffer}}\label{app.scheduling_policy_OptimalBuffer}
\noindent \textbf{Theorem \ref{theo.scheduling_policy_OptimalBuffer}}. The optimal scheduling probabilities for Single packet queues are given by
\begin{equation*}%\label{eq.scheduling_policy_OptimalBuffer}
\mu_i^S=\frac{\sqrt{w_i/p_i}}{\sum_{j=1}^N\sqrt{w_j/p_j}} , \forall i \; ,
\end{equation*}
and the performance of the Optimal Stationary Randomized Policy $R^S$ is
\begin{equation*}%\label{eq.EWSAoI_randomized_OptimalBuffer_final}
\mathbb{E}\left[J^{R^S}\right]=\frac{1}{N} \sum_{i=1}^N w_i \left(\frac{1}{\lambda_i}-1\right)+\frac{1}{N}\left( \sum_{i=1}^N \sqrt{\frac{w_i}{p_i}}\right)^2 .
\end{equation*}
Then, it follows that 
\begin{equation*}%\label{eq.Rand_OptimalBuffer}
\mathbb{E}\left[J^*\right]\leq \mathbb{E}\left[J^{R^S}\right]< 4\mathbb{E}\left[J^*\right] \; ,
\end{equation*}
where $\mathbb{E}\left[J^*\right]=\min_{\pi\in\Pi}\mathbb{E}\left[J^\pi\right]$ is the minimum AoI over the class of all admissible policies $\Pi$.

\begin{proof}
The scheduling probabilities $\{\mu_i^S\}_{i=1}^N$ are the argument that minimizes \eqref{eq.EWSAoI_randomized_OptimalBuffer}-\eqref{eq.EWSAoI_randomized_OptimalBuffer_2}. They can be easily found by using the fact that \eqref{eq.EWSAoI_randomized_OptimalBuffer} is convex in the interval $\mu_i\in(0,1]$. The detailed solution to \eqref{eq.EWSAoI_randomized_OptimalBuffer}-\eqref{eq.EWSAoI_randomized_OptimalBuffer_2} is provided in the technical report \cite[Appendix \ref{app.scheduling_policy_OptimalBuffer}]{TechRep}. 
Substituting $\{\mu_i^S\}_{i=1}^N$ in \eqref{eq.scheduling_policy_OptimalBuffer} into the objective function in \eqref{eq.EWSAoI_randomized_OptimalBuffer} gives \eqref{eq.EWSAoI_randomized_OptimalBuffer_final}. The derivation of the upper bound in \eqref{eq.Rand_OptimalBuffer} is shown next.
%\end{proof}
%
%The first term on the RHS of \eqref{eq.EWSAoI_randomized_OptimalBuffer_final} is associated with the time that each queue remains empty after a successful packet transmission. Consider queue $i$ in the slot that follows a successful packet transmission, the queue is empty with probability $1-\lambda_i$ and a packet arrives with probability $\lambda_i$. Hence, the number of slots until a packet arrival is geometric with parameter $\lambda_i$ and mean $1/\lambda_i-1$. 
%system time $z_i^S(t)$ of the HoL packets in the \emph{Single packet queues}. It follows from \eqref{eq.system_time_Optimal} that $z_i^S(t)$ is a renewal-reward process  with a geometric renewal interval with parameter $\lambda_i$. From the elementary renewal theorem for renewal-reward processes, we know that for every queue $i$
%The first term on the RHS of \eqref{eq.EWSAoI_randomized_Optimal_final} is associated with the system time $z_i^S(t)$ of the HoL packets in the \emph{Single packet queues}. It follows from \eqref{eq.system_time_Optimal} that $z_i^S(t)$ is a renewal-reward process \cite[Chapter 5]{DSP} with a geometric renewal interval with parameter $\lambda_i$. From the elementary renewal theorem for renewal-reward processes, we know that for every queue $i$
%\begin{equation}\label{eq.renewal_z}
%\lim_{T\rightarrow\infty}\frac{1}{T}\sum_{t=1}^{T}\mathbb{E}[z_i^S(t)]=\frac{\frac{1}{2}(\frac{2-\lambda_i}{\lambda_i^2}-\frac{1}{\lambda_i})}{\frac{1}{\lambda_i}}=\frac{1}{\lambda_i}-1 \; .
%\end{equation}
%The second term on the RHS of \eqref{eq.EWSAoI_randomized_OptimalBuffer_final} is associated with the time that the scheduling policy $R^S$ takes to successfully deliver packets, assuming that packets are always available at the queues, i.e. $\lambda_i=1,\forall i$. Hence, the expression in \eqref{eq.EWSAoI_randomized_OptimalBuffer_final} has one term for the queueing discipline and another for the scheduling policy. \emph{This separation is observed only for the case of \emph{Single packet queues}.} 
%
%\begin{corollary}\label{cor.Rand_OptimalBuffer}
%The Expected Weighted Sum AoI attained by the Optimal Stationary Randomized Policy $R^S\in\Pi_R$ is such that
%\begin{equation}\label{eq.Rand_OptimalBuffer}
%\mathbb{E}\left[J^*\right]\leq \mathbb{E}\left[J^{R^S}\right]< 4\mathbb{E}\left[J^*\right] \; ,
%\end{equation}
%where $\mathbb{E}\left[J^*\right]=\min_{\pi\in\Pi}\mathbb{E}\left[J^\pi\right]$ is the minimum AoI over the class of all admissible policies $\Pi$.
%\end{corollary}
%\begin{proof}

Consider the Randomized Policy $\tilde R$ with $\tilde{\mu}_i=\hat{q}_i^{L_B}/p_i,\forall i$. Substitute $\tilde{\mu}_i$ into the RHS of \eqref{eq.EWSAoI_randomized_OptimalBuffer} and denote the result as $\mathbb{E}[J^{\tilde R}]$. Comparing $L_B$ in \eqref{eq.LowerBound} with $\mathbb{E}[J^{\tilde R}]$ and noting from \eqref{eq.LowerBound_q} that $\hat{q}_i^{L_B}\leq \lambda_i$, gives that %for the particular Randomized Policy $R$ with $\tilde{\mu}_i=\hat{q}_i^{L_B}/p_i,\forall i$, we have
\begin{equation}%\label{eq.Rand_OptimalBuffer_1}
\mathbb{E}\left[J^{\tilde R}\right]\leq \frac{1}{N} \sum_{i=1}^N w_i \left(\frac{2}{p_i\tilde{\mu}_i}-1\right)<4L_B \; .
\end{equation}
By definition, we know that
\begin{equation}%\label{eq.Rand_OptimalBuffer_2}
L_B\leq\mathbb{E}[J^*]\leq\mathbb{E}[J^{R^S}]\leq\mathbb{E}[J^{\tilde R}] \; .
\end{equation}
Inequality \eqref{eq.Rand_OptimalBuffer} follows directly from \eqref{eq.Rand_OptimalBuffer_1} and \eqref{eq.Rand_OptimalBuffer_2}.
\end{proof}

==> body/12_appE_KKT_FIFO.tex <==
\section{Proof of Theorem \ref{theo.scheduling_policy_FIFOBuffer}}\label{app.scheduling_policy_FIFOBuffer}
\noindent \textbf{Theorem \ref{theo.scheduling_policy_FIFOBuffer}}. The optimal scheduling probabilities for the case of FIFO queues $\mu_i^F$ are given by Algorithm~\ref{alg.FIFO} when $\delta\rightarrow 0$.

\begin{algorithm}
\renewcommand{\thealgorithm}{2}
\caption{Randomized Policy for FIFO queue}
\begin{algorithmic}[1]
%  \Procedure{policy\_R}{$N,p_i,w_i,q_i$}
\State $\gamma_i \gets (\lambda_i+\delta)/p_i \; , \forall i \in \{1,2,\cdots,N\}$
%\State $\gamma_i \gets - g_i(\mu_i) \; , \forall i $
\State $\gamma \gets \max_{i}\{-g_i(\gamma_i)\}$ \Comment{where $g_i(.)$ is given in \eqref{eq.g}}
\State $\mu_i \gets \max\{\;\gamma_i\;;\;g_i^{-1}(-\gamma)\;\}$
\State $S \gets \mu_1+\mu_2+\cdots+\mu_N$
\While{$S<1$}
\State decrease $\gamma$ slightly
\State repeat steps 3 and 4 to update $\mu_i$ and $S$
%\State $\Gamma_i \gets  \; , \forall i$
%\State $\mu_i \gets (q_i / p_i)\max\{\,1\, ; \,\sqrt{\gamma_i/\gamma} \,\} \; , \forall i$
%\State $S \gets \mu_1+\mu_2+\cdots+\mu_N$
\EndWhile
\State \textbf{return} $\mu_i^F=\mu_i,\forall i$
%\State \textbf{return} $(\mu_1^*,\mu_2^*,\cdots,\mu_N^*,\gamma^*)$ %\Comment{Vector of probabilities}
%\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{proof}
To find the set of scheduling probabilities $\{\mu_i^F\}_{i=1}^N$ that solve the optimization problem \eqref{eq.Rand_FIFOBuff_1}-\eqref{eq.Rand_FIFOBuff_3}, we analyze the KKT Conditions. Let $\{\zeta_i\}_{i=1}^{N}$ be the KKT multipliers associated with the relaxation of \eqref{eq.Objective2_R} and $\gamma$ be the multiplier associated with the relaxation of \eqref{eq.Objective3_R}. Then, for $\zeta_i\geq 0, \forall i$, $\gamma\geq 0$ and $\mu_i\in(0,1], \forall i$, we define
\begin{align}
\mathcal{L}(\mu_i,&\zeta_i,\gamma)=\frac{1}{N}\sum_{i=1}^{N}\frac{w_i}{p_i\mu_i}+\nonumber\\
                  &+\sum_{i=1}^N\zeta_i\left(q_i-p_i\mu_i\right)+\gamma\left(\sum_{i=1}^N\mu_i -1\right) \; ,
\end{align}
and, otherwise, we define $\mathcal{L}(\mu_i,\zeta_i,\gamma)=+\infty$. Then, the KKT Conditions are
\begin{enumerate}[(i)]
\item Stationarity: $\nabla_{\mu_i}\mathcal{L}(\mu_i,\zeta_i,\gamma)=0$;
\item Complementary Slackness: $\gamma(\sum_{i=1}^N\mu_i-1)=0$;
\item Complementary Slackness: $\zeta_i(q_i-p_i\mu_i)=0, \forall i$;
\item Primal Feasibility: $p_i\mu_i \geq q_i \; , \forall i$, and $\sum_{i=1}^N\mu_i \leq 1$;
\item Dual Feasibility: $\zeta_i\geq 0, \forall i$, and $\gamma\geq 0$.
\end{enumerate}
Since $\mathcal{L}(\mu_i,\zeta_i,\gamma)$ is a \emph{convex function}, if there exists a vector $(\{\mu_i^*\}_{i=1}^N,\{\zeta_i^*\}_{i=1}^N,\gamma^*)$ that satisfies all KKT Conditions, then this vector is unique. Hence, the scheduling policy $R^*\in\Pi_R$ that optimizes \eqref{eq.Objective1_R}-\eqref{eq.Objective3_R} is also unique and is characterized by $\{\mu_i^*\}_{i=1}^N$. Next, we find the vector $(\{\mu_i^*\}_{i=1}^N,\{\zeta_i^*\}_{i=1}^N,\gamma^*)$.

To assess stationarity, $\nabla_{\mu_i}\mathcal{L}(\mu_i,\zeta_i,\gamma)=0$, we calculate the partial derivative of $\mathcal{L}(\mu_i,\zeta_i,\gamma)$ with respect to $\mu_i$. It follows from the derivative that
\begin{equation}\label{eq.KKT_equation1}
\frac{w_i}{Np_i\mu_i^2}+\zeta_ip_i=\gamma \; , \forall i \; .
\end{equation}

From complementary slackness, $\gamma(\sum_{i=1}^N\mu_i-1)=0$, we know that either $\gamma=0$ or $\sum_{i=1}^N\mu_i=1$. Equation \eqref{eq.KKT_equation1} shows that the value of $\gamma$ can only be zero if $\zeta_i=0$ and $\mu_i \rightarrow \infty$, which violates $\mu_i \in (0,1]$. Hence, we obtain
\begin{equation}\label{eq.KKT_equation2}
\gamma>0 \quad\mbox{and}\quad \sum_{i=1}^N\mu_i=1 \; . 
\end{equation}
Notice that $\sum_{i=1}^N\mu_i=1$ implies in $\mu_{idle}=0$.

%Combining \eqref{eq.KKT_equation1} and dual feasibility, $\zeta_i\geq 0$, we can write
%\begin{equation}\label{eq.KKT_equation3}
%\zeta_i=\frac{\gamma}{p_i}-\frac{w_i}{N(p_i\mu_i)^2}\geq 0 \;, \forall i 
%\end{equation}

Based on dual feasibility, $\zeta_i\geq 0$, we can separate nodes $i \in \{1,\cdots,N\}$ into two categories: nodes with $\zeta_i>0$ and nodes with $\zeta_i=0$.\\
\noindent\emph{Category 1)} node $i$ with $\zeta_i > 0$. It follows from complementary slackness, $\zeta_i(q_i-p_i\mu_i)=0$, that
\begin{equation}\label{eq.KKT_solution1}
\mu_i= \frac{q_i}{p_i} \; .
\end{equation}
Plugging this value of $\mu_i$ into \eqref{eq.KKT_equation1} gives the inequality $\zeta_ip_i=\gamma-\gamma_i> 0$, where we define the constant
\begin{equation}\label{eq.KKT_equation3}
\gamma_i:=\frac{w_ip_i}{Nq_i^2} \; .
\end{equation}
\noindent\emph{Category 2)} node $i$ with $\zeta_i=0$. It follows from \eqref{eq.KKT_equation1} that
\begin{equation}\label{eq.KKT_solution2}
\gamma=\gamma_i\left(\frac{q_i}{p_i\mu_i}\right)^2 \; \rightarrow \; \mu_i= \frac{q_i}{p_i}\sqrt{\frac{\gamma_i}{\gamma}}\; .
\end{equation}
In summary, for any fixed value of $\gamma>0$, the scheduling probability of node $i$ is
\begin{equation}\label{eq.mu}
\mu_i=\frac{q_i}{p_i}\max\left\{1 ; \sqrt{\frac{\gamma_i}{\gamma}}\right\} \; .
\end{equation}
Notice that for a decreasing value of $\gamma$, the probability $\mu_i$ remains fixed or increases. Our goal is to find the value of $\gamma^*$ that gives $\{\mu_i^*\}_{i=1}^N$ satisfying the condition $\sum_{i=1}^N\mu_i^*=1$.

\emph{Proposed algorithm to find }$\gamma^*$: start with $\gamma=\max \{\gamma_i\}$. Then, according to \eqref{eq.mu}, all nodes have $\mu_i=q_i/p_i$ and, by the feasibility condition in \eqref{eq.feasibility}, it follows that
\begin{equation}
\sum_{i=1}^N\mu_i=\sum_{i=1}^N\frac{q_i}{p_i}\leq 1 \; .
\end{equation}
Now, by gradually decreasing $\gamma$ and adjusting $\{\mu_i\}_{i=1}^N$ according to \eqref{eq.mu}, we can find the unique $\gamma^*$ that fulfills $\sum_{i=1}^N\mu_i^*=1$. The solution $\gamma^*$ exists since $\gamma \rightarrow 0$ implies in $\sum_{i=1}^N\mu_i \rightarrow \infty$. The uniqueness of $\gamma^*$ follows from the monotonicity of $\mu_i$ with respect to $\gamma$. This process is described in Algorithm~\ref{alg.KKT} and illustrated in Fig.~\ref{fig.Algorithm}.

Algorithm~\ref{alg.KKT} outputs the set of scheduling probabilities $\{\mu_i^*\}_{i=1}^N$ and the parameter $\gamma^*$. The set $\{\zeta_i^*\}_{i=1}^N$ is obtained using \eqref{eq.KKT_equation1}. Hence, the unique vector $(\{\mu_i^*\}_{i=1}^N,\{\zeta_i^*\}_{i=1}^N,\gamma^*)$ that solves the KKT Conditions is found.
\end{proof}

The auxiliary parameter $\delta>0$ is used to enforce a closed feasible set to the optimization problem in \eqref{eq.Rand_FIFOBuff_1}-\eqref{eq.Rand_FIFOBuff_3}. We exchange \eqref{eq.Rand_FIFOBuff_3} by $p_i\mu_i \geq \zeta_i +\delta,\forall i$, to ensure that Algorithm~\ref{alg.FIFO} always finds a unique solution to the KKT Conditions associated with \eqref{eq.Rand_FIFOBuff_1}-\eqref{eq.Rand_FIFOBuff_3} for any fixed (and arbitrarily small) value of $\delta$. Recall that when $p_i\mu_i \approx \zeta_i$ the AoI performance is poor. Hence, for most network configurations, the optimal scheduling probabilities $\{\mu_i^F\}_{i=1}^N$ are such that $p_i\mu_i^F$ and $\zeta_i$ are not close, meaning that small changes in $\delta$ should not affect the solution.

==> body/13_appF_PerformanceMW_S_old.tex <==
\section{Proof of Theorem \ref{theo.MW_bound_Optimal}}\label{app.MW_bound_Optimal}
\noindent \textbf{Theorem \ref{theo.MW_bound_Optimal}} (Performance Bounds for $MW^S$). Consider a network employing Single packet queues. The performance of the Max-Weight policy with $\beta_i=w_i[1/p_i\mu_i^S+1/\lambda_i-1],\forall i$, is such that
\begin{equation}%\label{eq.MW_bound_Optimal}
\mathbb{E}\left[J^{MW^S}\right]\leq\mathbb{E}\left[J^{R^S}\right]+\frac{1}{N}\sum_{i=1}^Nw_i\left(\frac{1}{\lambda_i}-1\right)\; ,
%\mathbb{E}\left[J^*\right]\leq \mathbb{E}\left[J^{MW^S}\right] < 6\mathbb{E}\left[J^*\right] \; ,
%L_B\leq \mathbb{E}\left[J^{MW^S}\right]\leq\mathbb{E}\left[J^{R^S}\right] \; ,
%\mathbb{E}\left[J^{MW^N}\right]&\leq\mathbb{E}\left[J^{R^N}\right]
%\mathbb{E}\left[J^{MW^F}\right]&\leq\mathbb{E}\left[J^{R^F}\right]
\end{equation}
where $\mu_i^S$ and $\mathbb{E}[J^{R^S}]$ are the optimal scheduling probability for the case of Single packet queues and the associated EWSAoI attained by $R^S$, respectively.

\begin{proof}
Consider stream $i$ from a network operating under the \emph{Single packet queue} discipline. In each slot $t$, a packet is transmitted, i.e. $u_i(t)=1$, if the stream is selected and it has a non-empty queue. Hence, packet transmissions $u_i(t)$ depend on the queue backlog. To decouple packet transmissions from the queue backlog, we create \emph{dummy packets} that can be transmitted without affecting the AoI. In particular, suppose that at time $t$ queue $i$ is selected and successfully transmits a packet with $z_i^S(t)=z$. Then, at the beginning of slot $t+1$, with probability $1-\lambda_i$ we place a \emph{dummy packet} with $z_i^S(t+1)=z+1$ at the HoL of the queue, otherwise we place a real packet with $z_i^S(t)=0$. %Notice that the value of $z_i^S(t)$ follows \eqref{eq.system_time_Optimal}. 
From that moment on, the behavior of dummy packets is indistinguishable from real packets. Notice that due to the choice of $z_i^S(t+1)=z+1$, when a dummy packet is delivered to the destination, it does not change the associated AoI. Moreover, the system time $z_i^S(t)$ is now defined at every slot $t$ following \eqref{eq.system_time_Optimal}. Next, we analyze the equivalent system with dummy packets.

The Age-Based Max-Weight policy minimizes the drift in \eqref{eq.LyapunovDrift_1}. Hence, any other policy $\pi \in \Pi$ yields a higher (or equal) value of $\Delta(\mathbb{S}(t))$. Consider the Stationary Randomized policy for Single packet queues defined in Sec.~\ref{sec.Random_OptimalBuffer} with scheduling probability $\mu_i^S$ and let 
%expected packet transmission from stream $i$ during slot $t$ given by
\begin{equation}\label{eq.uis}
\mathbb{E}\left[u_i(t)|\mathbb{S}(t)\right]=\mathbb{E}\left[u_i\right]=\mu_i^S \; .%\frac{1}{1/\mu_i^S+p_i/\lambda_i-p_i} \; .
\end{equation}
%Recall that a packet from stream $i$ is transmitted during slot $t$ if the stream is selected and the associated queue is non-empty. 
Substituting $\mathbb{E}\left[u_i\right]$ into the Lyapunov Drift gives 
\begin{align}\label{eq.drift_first}
\Delta(\mathbb{S}(t))\leq\frac{1}{N}\sum_{i=1}^N\beta_i-\frac{1}{N}\sum_{i=1}^N\beta_ip_i\left(h_i(t)-z_i^S(t)\right)\mathbb{E}\left[u_i\right] \; . 
\end{align}

Now, taking the expectation with respect to $\mathbb{S}(t)$ and then the time-average on the interval $t\in\{1,2,\cdots,T\}$ yields
\begin{align}
%\frac{\mathbb{E}\left[L(T+1)\right]}{T}&-\frac{\mathbb{E}\left[L(1)\right]}{T}\leq \frac{1}{N}\sum_{i=1}^N\beta_i+\nonumber\\
%-\frac{1}{TN}&\sum_{t=1}^T\sum_{i=1}^N\beta_ip_i\mathbb{E}\left[h_i(t)-z_i^S(t)\right]\mathbb{E}\left[u_i\right] \; .
\frac{\mathbb{E}\left[L(T+1)\right]}{T}-\frac{\mathbb{E}\left[L(1)\right]}{T}\leq \frac{1}{N}\sum_{i=1}^N\beta_i-\frac{1}{TN}\sum_{t=1}^T\sum_{i=1}^N\beta_ip_i\mathbb{E}\left[h_i(t)-z_i^S(t)\right]\mathbb{E}\left[u_i\right] \; .
\end{align}
Manipulating this expression, assigning $\beta_i=w_i/p_i\mathbb{E}\left[u_i\right]$ and taking the limit as $T\rightarrow\infty$, gives
\begin{align}\label{eq.MW_perf}
\mathbb{E}\left[J^{MW^S}\right]\leq&\frac{1}{N}\sum_{i=1}^N\frac{w_i}{p_i\mathbb{E}\left[u_i\right]}+\lim_{T\rightarrow\infty}\frac{1}{TN}\sum_{i=1}^N\sum_{t=1}^Tw_i\mathbb{E}\left[z_i^S(t)\right] \; .
\end{align}
From the evolution of $z_i^S(t)$ in \eqref{eq.system_time_Optimal}, we know that
\begin{equation}\label{eq.z_Singlequeue}
\lim_{T\rightarrow\infty}\frac{1}{TN}\sum_{i=1}^N\sum_{t=1}^Tw_i\mathbb{E}\left[z_i^S(t)\right]=\frac{1}{N}\sum_{i=1}^Nw_i\left(\frac{1}{\lambda_i}-1\right) \; .
\end{equation}
Substituting \eqref{eq.z_Singlequeue} and \eqref{eq.uis} into \eqref{eq.MW_perf} yields
\begin{align}\label{eq.MW_perf_2}
\mathbb{E}\left[J^{MW^S}\right]\leq&\frac{1}{N}\sum_{i=1}^N\frac{w_i}{p_i\mu_i^S}+\frac{2}{N}\sum_{i=1}^Nw_i\left(\frac{1}{\lambda_i}-1\right) \; .
\end{align}

For deriving the upper bound in \eqref{eq.MW_bound_Optimal}, consider the Optimal Stationary Randomized policy $R^S$. Substituting $\mu_i^S$ into \eqref{eq.EWSAoI_randomized_OptimalBuffer} and then comparing with \eqref{eq.MW_perf_2} gives
\begin{align}\label{eq.MW_perf_3}
\mathbb{E}\left[J^{MW^S}\right]\leq&\mathbb{E}\left[J^{R^S}\right]+\frac{1}{N}\sum_{i=1}^Nw_i\left(\frac{1}{\lambda_i}-1\right) \; .
\end{align}
Comparing the $L_B$ in \eqref{eq.LowerBound} with the second term on the RHS of \eqref{eq.MW_perf_3} and noting from \eqref{eq.LowerBound_q} that $\hat{q}_i^{L_B}\leq \lambda_i$ yields %for the particular Randomized policy $R$ with $\tilde{\mu}_i=\hat{q}_i^{L_B}/p_i,\forall i$, we have
\begin{equation}\label{eq.MW_OptimalBuffer_1}
\mathbb{E}\left[J^{MW^S}\right]\leq\mathbb{E}\left[J^{R^S}\right]+2L_B<6L_B \; .
\end{equation}
\end{proof}

%For deriving the upper bound in \eqref{eq.MW_bound_Optimal}, consider the Randomized policy $\tilde R$ with $\tilde{\mu}_i=\hat{q}_i^{L_B}/p_i,\forall i$. Substitute $\tilde{\mu}_i$ into the RHS of \eqref{eq.MW_perf_2} and denote the result as $\mathbb{E}[J^{\tilde R}]$. Comparing $L_B$ in \eqref{eq.LowerBound} with $\mathbb{E}[J^{\tilde R}]$ and noting from \eqref{eq.LowerBound_q} that $\hat{q}_i^{L_B}\leq \lambda_i$, gives that %for the particular Randomized policy $R$ with $\tilde{\mu}_i=\hat{q}_i^{L_B}/p_i,\forall i$, we have
%\begin{equation}\label{eq.MW_OptimalBuffer_1}
%\mathbb{E}\left[J^{\tilde R}\right]\leq \frac{1}{N} \sum_{i=1}^N w_i \left(\frac{3}{p_i\tilde{\mu}_i}-2\right)<6L_B \; .
%\end{equation}
%By definition, we know that
%\begin{equation}\label{eq.MW_OptimalBuffer_2}
%L_B\leq\mathbb{E}[J^*]\leq\mathbb{E}\left[J^{MW^S}\right]\leq\mathbb{E}[J^{\tilde R}] \; .
%\end{equation}
%Inequality \eqref{eq.MW_bound_Optimal} follows directly from \eqref{eq.MW_OptimalBuffer_1} and \eqref{eq.MW_OptimalBuffer_2}. 

==> body/9_appB_LowerBound_wrong.tex <==
\section{Proof of Theorem \ref{theo.LowerBound}}\label{app.LowerBound}
\noindent \textbf{Theorem \ref{theo.LowerBound}} (Lower Bound). For any given network with parameters $(N,p_i,\lambda_i,w_i)$ and an arbitrary queueing discipline, the optimization problem in \eqref{eq.LowerBound_1}-\eqref{eq.LowerBound_3} provides a lower bound on the AoI minimization problem, namely $L_B\leq\mathbb{E}[J^*]$. The unique solution to \eqref{eq.LowerBound_1}-\eqref{eq.LowerBound_3} is given by
\begin{equation*}%\label{eq.LowerBound_q}
\hat{q}_i^{L_B}=\min{\left\{\lambda_i,\sqrt{\frac{w_ip_i}{2N\gamma^*}}\right\}}, \forall i \; ,
\end{equation*}
where $\gamma^*$ yields from Algorithm~\ref{alg.LowerBound}. The lower bound is given by 
\begin{equation*}
L_B=\frac{1}{2N}\sum_{i=1}^Nw_i\left(\frac{1}{\hat{q}_i^{L_B}}+1\right) \; .
\end{equation*}

%\begin{algorithm}
%\renewcommand{\thealgorithm}{1}
%\caption{Maximum Throughput for Lower Bound}
%\begin{algorithmic}[1]
%\State $\gamma \gets \max_i{\{w_ip_i/\lambda_i^2\}}$
%\State $\gamma \gets \max{\{\gamma ; (\sum_{i=1}^M\sqrt{w_i/p_i})^2\}}/2M$
%\State $q_i \gets \min{\{\lambda_i,\sqrt{w_ip_i/2M\gamma}\}}, \forall i$
%\State $S \gets \sum_{i=1}^Mq_i/p_i$
%\While{$S<1$ \textbf{and} $\gamma>0$}
%\State decrease $\gamma$ slightly
%\State repeat steps 3 and 4 to update $q_i$ and $S$
%\EndWhile
%%\State $\gamma^*=\gamma$ and $\hat{q}_i^{L_B}=q_i,\forall i$
%\State \textbf{return} $\gamma^*=\gamma$ and $\hat{q}_i^{L_B}=q_i,\forall i$
%%\EndProcedure
%\end{algorithmic}
%\end{algorithm}

%\begin{algorithm}
%\renewcommand{\thealgorithm}{1}
%\caption{Maximum Throughput for Lower Bound}
%\begin{algorithmic}[1]
%\State $\tilde{\gamma} \gets (\sum_{i=1}^M\sqrt{w_i/p_i})^2/(2M)$ and $\gamma_i \gets w_ip_i/2M\lambda_i^2 , \forall i$
%\State $\gamma \gets \max\{\tilde{\gamma};\gamma_i\}$
%%\State $\gamma \gets \max{\{\gamma ; (\sum_{i=1}^M\sqrt{w_i/p_i})^2\}}/2M$
%\State $q_i \gets \lambda_i\min\{1 ; \sqrt{\gamma_i/\gamma}\} , \forall i$
%\State $S \gets \sum_{i=1}^Mq_i/p_i$
%\While{$S<1$ \textbf{and} $\gamma\geq\min\{\gamma_i\}$}
%\State decrease $\gamma$ slightly
%\State repeat steps 4 and 5 to update $q_i$ and $S$
%\EndWhile
%%\State $\gamma^*=\gamma$ and $\hat{q}_i^{L_B}=q_i,\forall i$
%\State \textbf{if} $\gamma<\min\{\gamma_i\}$ \textbf{then} $\gamma\gets 0$ and $q_i\gets \lambda_i,\forall i$ \textbf{end if}
%%\If{$\gamma<\min\{\gamma_i\}$}
%%State $\gamma=0$
%%\EndIf
%\State \textbf{return} $\gamma^*=\gamma$ and $\hat{q}_i^{L_B}=q_i,\forall i$
%%\EndProcedure
%\end{algorithmic}
%\end{algorithm}

\begin{algorithm}
\renewcommand{\thealgorithm}{1}
\caption{Maximum Throughput for Lower Bound}
\begin{algorithmic}[1]
\State $\tilde{\gamma} \gets (\sum_{i=1}^N\sqrt{w_i/p_i})^2/(2N)$ and $\gamma_i \gets w_ip_i/2N\lambda_i^2 , \forall i$
\State $\gamma \gets \max\{\tilde{\gamma};\gamma_i\}$
%\State $\gamma \gets \max{\{\gamma ; (\sum_{i=1}^N\sqrt{w_i/p_i})^2\}}/2N$
\State $q_i \gets \lambda_i\min\{1 ; \sqrt{\gamma_i/\gamma}\} , \forall i$
\State $S \gets \sum_{i=1}^Nq_i/p_i$
\While{$S<1$ \textbf{and} $\gamma>0$}
\State decrease $\gamma$ slightly
\State repeat steps 4 and 5 to update $q_i$ and $S$
\EndWhile
%\State $\gamma^*=\gamma$ and $\hat{q}_i^{L_B}=q_i,\forall i$
%\State \textbf{if} $\gamma<\min\{\gamma_i\}$ \textbf{then} $\gamma\gets 0$ and $q_i\gets \lambda_i,\forall i$ \textbf{end if}
%\If{$\gamma<\min\{\gamma_i\}$}
%State $\gamma=0$
%\EndIf
\State \textbf{return} $\gamma^*=\gamma$ and $\hat{q}_i^{L_B}=q_i,\forall i$
%\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{proof}
Consider a network with parameters $(N,p_i,\lambda_i,w_i)$ and an arbitrary queueing discipline. First, we show that \eqref{eq.LowerBound_1}-\eqref{eq.LowerBound_3} provides a lower bound $L_B$ on the AoI minimization problem $\mathbb{E}[J^*]=\min_{\pi\in\Pi}\mathbb{E}\left[J^\pi\right]$, then we find the unique solution to \eqref{eq.LowerBound_1}-\eqref{eq.LowerBound_3} by analyzing its KKT Conditions. The optimization problem in \eqref{eq.LowerBound_1}-\eqref{eq.LowerBound_3} is rewritten below for convenience.
\begin{subequations}
\begin{align*}
L_B=&\min_{\pi\in\Pi}\left\{\frac{1}{2N}\sum_{i=1}^Nw_i\left(\frac{1}{\hat{q}_i^{\pi}}+1\right)\right\} \\
\mbox{s.t. } &\textstyle\sum_{i=1}^N \hat{q}_i^{\pi}/p_i \leq 1 \; ;\\
&\hat{q}_i^{\pi} \leq \lambda_i , \forall i \; .%\label{eq.LowerBound_3_}
\end{align*}
\end{subequations}
%The expression in \eqref{eq.sum} is central for this proof and is rewritten below for convenience.
%\begin{align*}
%\frac{1}{T}\sum_{t=1}^{T}h_i(t)&=\frac{1}{2}\left[\frac{D_i(T)}{T}\;\frac{1}{D_i(T)}\sum_{m=1}^{D_i(T)} \left(I_i^2[m]+2z_i[m-1]I_i[m]\right)+\frac{R_i^2}{T}+2\frac{z_i[D_i(T)]R_i}{T}+1\right] \; .
%\end{align*}

Consider the expression for the time-average AoI associated with destination $i$ in \eqref{eq.sum}, which is valid for any admissible policy $\pi\in\Pi$ and time-horizon $T$. Substituting the non-negative terms $z_i[m-1]I_i[m]$ and $z_i[D_i(T)]R_i$ by zero, employing the sample mean operator $\mathbb{\bar{M}}$ to $I_i^2[m]$ and then applying Jensen's inequality $\mathbb{\bar{M}}[I_i^2]\geq(\mathbb{\bar{M}}[I_i])^2$, we obtain
\begin{equation}\label{eq.sum2}
\frac{1}{T}\sum_{t=1}^{T}h_i(t) \geq  \frac{1}{2}\left(\frac{D_i(T)}{T}\left(\bar{\mathbb{M}}[I_i]\right)^2+\frac{R_i^2}{T}+1\right) \; .
\end{equation}
Substituting \eqref{eq.relation_throughput} into \eqref{eq.sum2}, gives
\begin{equation}\label{eq.sum3}
\frac{1}{T}\sum_{t=1}^{T}h_i(t) \geq  \frac{1}{2}\left(\frac{1}{T}\frac{(T-R_i)^2}{D_i(T)}+\frac{R_i^2}{T}+1\right) \; .
\end{equation}
By minimizing the LHS of \eqref{eq.sum3} analytically with respect to the variable $R_i$, we have
\begin{equation}\label{eq.sum4}
\frac{1}{T}\sum_{t=1}^{T}h_i(t) \geq  \frac{1}{2}\left(\frac{T}{D_i(T)+1}+1\right) \; .
\end{equation}
Taking the expectation of \eqref{eq.sum4} and applying Jensen's inequality, yields
\begin{equation}\label{eq.sum5}
\frac{1}{T}\sum_{t=1}^{T}\mathbb{E}\left[h_i(t)\right] \geq  \frac{1}{2}\left(\frac{1}{\mathbb{E}\left[\displaystyle\frac{D_i(T)}{T}\right]+\displaystyle\frac{1}{T}}+1\right) \; .
\end{equation}
Applying the limit $T\rightarrow\infty$ to \eqref{eq.sum5} and using the definition of throughput in \eqref{eq.throughput}, gives
\begin{equation}\label{eq.sum6}
\lim_{T\rightarrow\infty}\frac{1}{T}\sum_{t=1}^{T}\mathbb{E}\left[h_i(t)\right] \geq  \frac{1}{2}\left(\frac{1}{\hat{q}_i^\pi}+1\right) \; .
\end{equation}
Substituting \eqref{eq.sum6} into the objective function in \eqref{eq.Objective_1}, yields 
\begin{align}\label{eq.obj1}
\mathbb{E}\left[J^{\pi}\right]=&\lim_{T\rightarrow\infty}\frac{1}{N}\sum_{i=1}^N\frac{w_i}{T}\sum_{t=1}^{T}\mathbb{E}\left[ h_i(t) \right]\nonumber \\
\geq&\frac{1}{2N}\sum_{i=1}^N w_i \left(\frac{1}{\hat{q}_i^\pi}+1\right)\; .
\end{align}
Inequality \eqref{eq.obj1} is valid for any admissible policy $\pi\in\Pi$. Notice that the RHS of \eqref{eq.obj1} depends only on the network's long-term throughput $\{\hat{q}_i^{\pi}\}_{i=1}^N$. Adding to \eqref{eq.obj1} the two necessary conditions for the long-term throughput in \eqref{eq.throughput_condition1} and \eqref{eq.throughput_condition2}, and then minimizing the resulting problem over all policies in $\Pi$, yields $\mathbb{E}[J^*]=\min_{\pi\in\Pi}\mathbb{E}\left[J^\pi\right]\geq L_B$ where $L_B$ is given by \eqref{eq.LowerBound_1}-\eqref{eq.LowerBound_3}.

After showing that \eqref{eq.LowerBound_1}-\eqref{eq.LowerBound_3} provides a lower bound on the AoI minimization problem, we find the unique set of network's long-term throughput $\{\hat{q}_i^{L_B}\}_{i=1}^N$ that solves \eqref{eq.LowerBound_1}-\eqref{eq.LowerBound_3} by analyzing its KKT Conditions. Let $\gamma$ be the KKT multiplier associated with the relaxation of $\sum_{i=1}^N \hat{q}_i^{\pi}/p_i \leq 1$ and $\{\lambda_i\}_{i=1}^{N}$ be the KKT multipliers associated with the relaxation of $\hat{q}_i^{\pi} \leq \lambda_i , \forall i$. Then, for $\gamma\geq 0$ , $\lambda_i\geq 0$ and $\hat{q}_i^\pi\in(0,1], \forall i$, we define
\begin{align}
\mathcal{L}(\hat{q}_i^\pi,&\lambda_i,\gamma)=\frac{1}{2N}\sum_{i=1}^Nw_i\left(\frac{1}{\hat{q}_i^\pi}+1\right)+\sum_{i=1}^N\lambda_i\left(\hat{q}_i^\pi-\lambda_i\right)+\gamma\left(\sum_{i=1}^N\frac{\hat{q}_i^{\pi}}{p_i}-1\right) \; ,
\end{align}
and, otherwise, we define $\mathcal{L}(\hat{q}_i^\pi,\lambda_i,\gamma)=+\infty$. Then, the KKT Conditions are
\begin{enumerate}[(i)]
\item Stationarity: $\nabla_{\hat{q}_i^\pi}\mathcal{L}(\hat{q}_i^\pi,\lambda_i,\gamma)=0$;
\item Complementary Slackness: $\gamma(\sum_{i=1}^N\hat{q}_i^{\pi}/p_i-1)=0$;
\item Complementary Slackness: $\lambda_i(\hat{q}_i^\pi-\lambda_i)=0, \forall i$;
\item Primal Feasibility: $\hat{q}_i^{\pi} \leq \lambda_i , \forall i$, and $\sum_{i=1}^N \hat{q}_i^{\pi}/p_i \leq 1$;
\item Dual Feasibility: $\lambda_i\geq 0, \forall i$, and $\gamma\geq 0$.
\end{enumerate}
Since $\mathcal{L}(\hat{q}_i^\pi,\lambda_i,\gamma)$ is a \emph{convex function}, if there exists a vector $(\{\hat{q}_i^{L_B}\}_{i=1}^N,\{\lambda_i^*\}_{i=1}^N,\gamma^*)$ that satisfies all KKT Conditions, then this vector is unique. %Hence, the scheduling policy $R^*\in\Pi_R$ that optimizes \eqref{eq.Objective1_R}-\eqref{eq.Objective3_R} is also unique and is characterized by $\{\hat{q}_i^{L_B}\}_{i=1}^N$. 
Next, we find the vector $(\{\hat{q}_i^{L_B}\}_{i=1}^N,\{\lambda_i^*\}_{i=1}^N,\gamma^*)$.

To assess stationarity, $\nabla_{\hat{q}_i^\pi}\mathcal{L}(\hat{q}_i^\pi,\lambda_i,\gamma)=0$, we calculate the partial derivative of $\mathcal{L}(\hat{q}_i^\pi,\lambda_i,\gamma)$ with respect to $\hat{q}_i^\pi$, which gives%. It follows from the derivative that
\begin{equation}\label{eq.KKT_equation1}
-\frac{w_ip_i}{2N(\hat{q}_i^\pi)^2}+\lambda_ip_i+\gamma=0 \; , \forall i \; .
\end{equation}

From complementary slackness, $\gamma(\sum_{i=1}^N\hat{q}_i^{\pi}/p_i-1)=0$, we know that either $\gamma=0$ or $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$. First, we consider the case $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$. Based on dual feasibility, $\lambda_i\geq 0$, we can separate streams $i \in \{1,\cdots,N\}$ into two categories: streams with $\lambda_i>0$ and streams with $\lambda_i=0$.\\
\noindent\emph{Category 1)} stream $i$ with $\lambda_i > 0$. It follows from complementary slackness, $\lambda_i(\hat{q}_i^\pi-\lambda_i)=0$, that $\hat{q}_i^\pi= \lambda_i$. Plugging this value of $\hat{q}_i^\pi$ into \eqref{eq.KKT_equation1} gives the inequality $\lambda_ip_i=\gamma_i-\gamma> 0$, where we define the constant
\begin{equation}\label{eq.KKT_equation3}
\gamma_i:=\frac{w_ip_i}{2N\lambda_i^2} \; .
\end{equation}
\noindent\emph{Category 2)} stream $i$ with $\lambda_i=0$. It follows from \eqref{eq.KKT_equation1} that
\begin{equation}\label{eq.KKT_solution2}
\gamma=\gamma_i\left(\frac{\lambda_i}{\hat{q}_i^\pi}\right)^2 \Rightarrow \; \hat{q}_i^\pi= \lambda_i\sqrt{\frac{\gamma_i}{\gamma}}\; , \mbox{for } \gamma_i-\gamma\leq 0 \; .
\end{equation}
Hence, for any fixed value of $\gamma\geq 0$, if $\gamma\geq\gamma_i$ then stream $i$ is in Category 2, otherwise, stream $i$ is in Category 1. Moreover, the values of $\lambda_i$ and $\hat{q}_i^\pi$ associated with stream $i$, in either Category, can be expressed as
\begin{align}
\lambda_i=\max\left\{0 ; \frac{\gamma_i-\gamma}{p_i}\right\} ,\forall i \; . \label{eq.lambda} \\
\hat{q}_i^\pi=\lambda_i\min\left\{1 ; \sqrt{\frac{\gamma_i}{\gamma}}\right\} ,\forall i \; . \label{eq.mu}
\end{align}
Notice that when $\gamma>\max\{\gamma_i\}$, then all streams are in Category 2 and $\hat{q}_i^\pi< \lambda_i,\forall i$. By decreasing the value of $\gamma$ gradually, the throughput $\hat{q}_i^\pi$ of each stream $i$ in \eqref{eq.mu} either increases or remain fixed at $\lambda_i$. Our goal is to find the value of $\gamma^*$ which yields $\{\hat{q}_i^{\pi}\}_{i=1}^N$ satisfying the condition $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$. Suppose this condition is satisfied when $\gamma>\max\{\gamma_i\}$, with all streams in Category 2, then it follows that
\begin{align}
&\sum_{i=1}^N\frac{\hat{q}_i^\pi}{p_i}=\sum_{i=1}^N\frac{\lambda_i}{p_i}\sqrt{\frac{\gamma_i}{\gamma}}=\frac{1}{\sqrt{2N\gamma}}\sum_{i=1}^N\sqrt{\frac{w_i}{p_i}}=1 \Rightarrow\nonumber\\
& \Rightarrow \gamma^*=\tilde{\gamma}:=\frac{1}{2N}\left(\sum_{i=1}^N\sqrt{\frac{w_i}{p_i}}\right)^2 \; ,
\label{eq.condition1}
\end{align}
where $\tilde{\gamma}$ is a fixed constant and the solution is unique $\gamma^*=\tilde{\gamma}$.

Alternatively, suppose that $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$ is satisfied when $\min\{\gamma_i\}\leq\gamma\leq\max\{\gamma_i\}$, with some streams in Category 1 and others in Category 2. To find $\gamma^*$, we start with $\gamma=\max\{\gamma_i\}$ and gradually decrease $\gamma$, adjusting $\{\hat{q}_i^\pi\}_{i=1}^N$ according to \eqref{eq.mu} until we reach $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$. The uniqueness of $\gamma^*$ follows from the monotonicity of $\hat{q}_i^\pi$ with respect to $\gamma$ in \eqref{eq.mu}.

Another possibility is for $\gamma$ to reach a value lower than $\min\{\gamma_i\}$ and still result in $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i<1$. Notice from \eqref{eq.mu} that when $\gamma<\min\{\gamma_i\}$, then all streams are in Category 1 and have maximum throughputs, namely $\hat{q}_i^{\pi}=\lambda_i,\forall i$. It follows that $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=\sum_{i=1}^N\lambda_i/p_i<1$, in which case the condition $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$ cannot be satisfied for any value of $\gamma\geq 0$. Hence, from complementary slackness, $\gamma(\sum_{i=1}^N\hat{q}_i^{\pi}/p_i-1)=0$, we have the unique solution $\gamma^*=0$.

\emph{Proposed algorithm to find }$\gamma^*$ that solves the KKT Conditions: start with $\gamma=\max\{\gamma_i;\tilde{\gamma}\}$. Then, compute $\{\hat{q}_i^\pi\}_{i=1}^N$ using \eqref{eq.mu} and verify if the condition $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$ is satisfied. If $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i<1$, then gradually decrease $\gamma$ and repeat the procedure. Stop when $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$ or when $\gamma<\min\{\gamma_i\}$. If $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$ holds, then assign $\gamma^*\leftarrow\gamma$. Otherwise, if $\gamma<\min\{\gamma_i\}$ holds, then assign $\gamma^*\leftarrow 0$. The solution to the KKT Conditions is given by $\gamma^*$ and the associated $\lambda_i^*$ and $\hat{q}_i^{L_B}$ obtained by substituting $\gamma^*$ into \eqref{eq.lambda} and \eqref{eq.mu}, respectively.

It is evident from the proposed algorithm that for any given network with parameters $(N,p_i,\lambda_i,w_i)$ and an arbitrary queueing discipline, the solution to the KKT Conditions, $(\{\hat{q}_i^{L_B}\}_{i=1}^N,\{\lambda_i^*\}_{i=1}^N,\gamma^*)$, exists and is unique. The proposed algorithm is described using pseudocode in Algorithm~\ref{alg.LowerBound}.


%Summary of proif the RHS of \eqref{eq.condition1} is larger than $\max\{\gamma_i\}$, then $\gamma^*$ is given by \eqref{eq.condition1}, otherwise the value of $\gamma^*$ is obtained using the procedure described above in which $\gamma$ is gradually decreased until $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$. In both cases, 

%Another possibility is for $\gamma$ to reach zero and $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i<1$. From \eqref{eq.mu}, it follows that when $\gamma\rightarrow 0$, we have $\hat{q}_i^{\pi}=\lambda_i,\forall i$. Hence, this is the first case discussed in this proof, where $\gamma=0$ and $\sum_{i=1}^N\lambda_i/p_i<1$, for which the optimal solution to the KKT Conditions was given by $\hat{q}_i^{L_B}=\lambda_i,\forall i$, $\lambda_i^*=w_i/(2N\lambda_i^2),\forall i$ and $\gamma^*=0$.

%\textbf{First, we consider the case} $\gamma=0$. Equation \eqref{eq.KKT_equation1} shows that if $\gamma=0$, then $\lambda_i>0,\forall i$. Hence, from complementary slackness, $\lambda_i(\hat{q}_i^\pi-\lambda_i)=0, \forall i$, we know that $\hat{q}_i^\pi=\lambda_i,\forall i$. However, this can only hold if primal feasibility is satisfied, namely
%\begin{equation}\label{eq.KKT_equation2}
%\sum_{i=1}^N \frac{\lambda_i}{p_i} \leq 1 \; .
%\end{equation}
%As a result, when the parameters of the network are such that inequality \eqref{eq.KKT_equation2} is fulfilled, then a solution to the KKT Conditions is given by $\hat{q}_i^{L_B}=\lambda_i,\forall i$, $\lambda_i^*=w_i/(2N\lambda_i^2),\forall i$ and $\gamma^*=0$.


%\newpage
%
%
%
%
%Then, according to \eqref{eq.mu}, all streams have $\hat{q}_i^\pi\leq \lambda_i$ and, by the feasibility condition in \eqref{eq.feasibility}, it follows that
%\begin{equation}
%\sum_{i=1}^N\mu_i=\sum_{i=1}^N\frac{q_i}{p_i}\leq 1 \; .
%\end{equation}
%Now, by gradually decreasing $\gamma$ and adjusting $\{\hat{q}_i^\pi\}_{i=1}^N$ according to \eqref{eq.mu}, we can find the unique $\gamma^*$ that fulfills $\sum_{i=1}^N\mu_i^*=1$. The solution $\gamma^*$ exists since $\gamma \rightarrow 0$ implies in $\sum_{i=1}^N\mu_i \rightarrow \infty$. The uniqueness of $\gamma^*$ follows from the monotonicity of $\hat{q}_i^\pi$ with respect to $\gamma$. This process is described in Algorithm~\ref{alg.LowerBound}. %and illustrated in Fig.~\ref{fig.Algorithm}.
%
%From the and $\hat{q}_i^\pi \rightarrow \infty$, which violates $\hat{q}_i^\pi \in (0,1]$. Hence, we obtain
%\begin{equation}%label{eq.KKT_equation2}
%\gamma>0 \quad\mbox{and}\quad \sum_{i=1}^N\mu_i=1 \; . 
%\end{equation}
%Notice that $\sum_{i=1}^N\mu_i=1$ implies in $\mu_{idle}=0$.
%
%
%Algorithm~\ref{alg.LowerBound} outputs the set of scheduling probabilities $\{\hat{q}_i^{L_B}\}_{i=1}^N$ and the parameter $\gamma^*$. The set $\{\lambda_i^*\}_{i=1}^N$ is obtained using \eqref{eq.KKT_equation1}. Hence, the unique vector $(\{\hat{q}_i^{L_B}\}_{i=1}^N,\{\lambda_i^*\}_{i=1}^N,\gamma^*)$ that solves the KKT Conditions is found.
%
%
%
%
%
%we start with a high enough value of $\gamma$ and continually. 
%
%which gives $\{\hat{q}_i^{\pi}\}_{i=1}^N$ satisfying the condition $\sum_{i=1}^N\hat{q}_i^{\pi}/p_i=1$. One possibility is to find a large $\gamma$ and all streams in Category 2 with $\lambda_i=0\forall i$. In this case, $\hat{q}_i^\pi$ is given by \eqref{eq.KKT_solution2}
%
% vector $(\{\hat{q}_i^{L_B}\}_{i=1}^N,\{\lambda_i^*\}_{i=1}^N,\gamma^*)$ that satisfies all KKT Conditions. We know that
%
%
%
%
%
%
%
%
%
%
%Hence, there is an unique value of $\gamma^*$ which gives $\{\hat{q}_i^{L_B}\}_{i=1}^N$ satisfying the condition $\sum_{i=1}^N\hat{q}_i^{L_B}/p_i=1$
%
%Our goal is to find the value of $\gamma^*$ which gives $\{\hat{q}_i^{L_B}\}_{i=1}^N$ satisfying the condition
%\begin{equation}
%\sum_{i=1}^N\frac{\hat{q}_i^{L_B}}{p_i}=\min\left\{1;\sum_{i=1}^N\frac{\lambda_i}{p_i} \right\}
%\end{equation}
%It is also possible that 
%
%One extreme case occurs when $\sum_{i=1}^N\hat{q}_i^{L_B}/p_i=1$ can never be achieved 
%
%$\gamma^*$ is such that $q$
%
%\emph{Proposed algorithm to find }$\gamma^*$ that solves the KKT Conditions: start with $\gamma=\max \{\gamma_i\}$. Then, according to \eqref{eq.mu}, all streams have $\hat{q}_i^\pi\leq \lambda_i$ and, by the feasibility condition in \eqref{eq.feasibility}, it follows that
%\begin{equation}
%\sum_{i=1}^N\mu_i=\sum_{i=1}^N\frac{q_i}{p_i}\leq 1 \; .
%\end{equation}
%Now, by gradually decreasing $\gamma$ and adjusting $\{\hat{q}_i^\pi\}_{i=1}^N$ according to \eqref{eq.mu}, we can find the unique $\gamma^*$ that fulfills $\sum_{i=1}^N\mu_i^*=1$. The solution $\gamma^*$ exists since $\gamma \rightarrow 0$ implies in $\sum_{i=1}^N\mu_i \rightarrow \infty$. The uniqueness of $\gamma^*$ follows from the monotonicity of $\hat{q}_i^\pi$ with respect to $\gamma$. This process is described in Algorithm~\ref{alg.LowerBound}. %and illustrated in Fig.~\ref{fig.Algorithm}.
%
%From the and $\hat{q}_i^\pi \rightarrow \infty$, which violates $\hat{q}_i^\pi \in (0,1]$. Hence, we obtain
%\begin{equation}%label{eq.KKT_equation2}
%\gamma>0 \quad\mbox{and}\quad \sum_{i=1}^N\mu_i=1 \; . 
%\end{equation}
%Notice that $\sum_{i=1}^N\mu_i=1$ implies in $\mu_{idle}=0$.
%
%
%Algorithm~\ref{alg.LowerBound} outputs the set of scheduling probabilities $\{\hat{q}_i^{L_B}\}_{i=1}^N$ and the parameter $\gamma^*$. The set $\{\lambda_i^*\}_{i=1}^N$ is obtained using \eqref{eq.KKT_equation1}. Hence, the unique vector $(\{\hat{q}_i^{L_B}\}_{i=1}^N,\{\lambda_i^*\}_{i=1}^N,\gamma^*)$ that solves the KKT Conditions is found.

\end{proof}
